Fine-Grained Object Detection over Scientific Document Images with Region Embeddings

We study the problem of object detection over scanned images of scientific documents. We consider images that contain objects of varying aspect ratios and sizes and range from coarse elements such as tables and figures to fine elements such as equations and section headers. We find that current object detectors fail to produce properly localized region proposals over such page objects. We revisit the original R-CNN model and present a method for generating fine-grained proposals over document elements. We also present a region embedding model that uses the convolutional maps of a proposal's neighbors as context to produce an embedding for each proposal. This region embedding is able to capture the semantic relationships between a target region and its surrounding context. Our end-to-end model produces an embedding for each proposal, then classifies each proposal by using a multi-head attention model that attends to the most important neighbors of a proposal. To evaluate our model, we collect and annotate a dataset of publications from heterogeneous journals. We show that our model, referred to as Attentive-RCNN, yields a 17% mAP improvement compared to standard object detection models.

==> ICDAR.tex <==
Previous page object detection models generally focus on a single class instead of detecting and classifying all objects on a page. The ICDAR POD 2017 challenge was one such competition, with separate challenges for classifying tables, figures, and equations, as well as all three. As we do not have access to the actual test set, we partition the training set into train/test splits, and train using the same optimized hyperparameters as the Geoscience dataset for all models.


==> classification.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ |c |c |c| c| c| c| c| c|c |c |c| c| c| c|c |c| c| c| c| c| c|c |c |c| c| c| c | c |c| c| c| c| c| c|c |c |c| c| c| c|}
\hline
& \multicolumn{3}{c|}{Body Text} & \multicolumn{3}{c|}{Equation} & \multicolumn{3}{c|}{Figure} & \multicolumn{3}{c|}{Figure Caption} & \multicolumn{3}{c|}{Other} & \multicolumn{3}{c|}{Page Footer} & \multicolumn{3}{c|}{Page Header} & \multicolumn{3}{c|}{Reference Text}& \multicolumn{3}{c|}{Section Header} & \multicolumn{3}{c|}{Table} & \multicolumn{3}{c|}{Table Caption} & \multicolumn{3}{c|}{All} \\

& P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ \\
\hline
Faster-RCNN & 6,578 & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
\hline
R-CNN & 1,258 & 272 & 276 & 274 & 64 & 206 & 533 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
+ Postprocessing & 1,258 & 272 & 276 & 274 & 64 & 206 & 533 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
\hline
Attentive-RCNN & 1,258 & 272 & 276 & 274 & 64 & 206 & 533 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
+ Postprocessing & 1,258 & 272 & 276 & 274 & 64 & 206 & 533 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
\hline
\end{tabular}}
\caption{ Classification results given proposals for which all models have high IOU ($> 0.8$)}
\label{table:classificationrcnnf1}
\end{center}
\end{table*}

\begin{table*}[t]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ |c |c |c| c| c| c| c| c|c |c |c| c| c| c|c |c| c| c| c| c| c|c |c |c| c| c| c | c |c| c| c| c| c| c|c |c |c| c| c| c|}
\hline
& \multicolumn{3}{c|}{Body Text} & \multicolumn{3}{c|}{Equation} & \multicolumn{3}{c|}{Figure} & \multicolumn{3}{c|}{Figure Caption} & \multicolumn{3}{c|}{Other} & \multicolumn{3}{c|}{Page Footer} & \multicolumn{3}{c|}{Page Header} & \multicolumn{3}{c|}{Reference Text}& \multicolumn{3}{c|}{Section Header} & \multicolumn{3}{c|}{Table} & \multicolumn{3}{c|}{Table Caption} & \multicolumn{3}{c|}{All} \\

& P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ \\
\hline
Faster-RCNN & 6,578 & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
\hline
R-CNN & 1,258 & 272 & 276 & 274 & 64 & 206 & 533 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
+ Postprocessing & 1,258 & 272 & 276 & 274 & 64 & 206 & 533 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
\hline
Attentive-RCNN & 1,258 & 272 & 276 & 274 & 64 & 206 & 533 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
+ Postprocessing & 1,258 & 272 & 276 & 274 & 64 & 206 & 533 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646  & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646 & 1 & 1\\
\hline
\end{tabular}}
\caption{Classification results for which grid proposals have  high IOU ($>0.8$)}
\label{table:classificationgridf1}
\end{center}
\end{table*}

==> dataset.tex <==
Because we are interested in detecting more classes of object on a page than any prior page object detection dataset, we annotate a collection of 2466 images from Geoscience papers provided by the GeoDeepDive project. We divide the pages into an 84:16 train/test split. We provide the class object counts of the train and test partitions in Table \ref{table:class_counts}.

The dataset is composed of single page images randomly selected from documents, with no pdf metadata provided for each image. As a result, metadata objects cannot be used to segment or classify anything on the page: visual information is all that is provided. Documents are collected from a variety of source conferences and journals with heterogenous layouts. Furthermore, documents can date as far back as 1970, and thus are sometimes not typeset. Some documents are scanned and not rendered, and consequently the quality of the text on the page itself varies greatly.

The Other class is defined as objects in the page that do not contribute scientific content and can be ignored. Wherever possible, annotators were told to create a one to one correspondence between tables/figures and their respective captions, such that groups of tables/figures associated with a single caption are labelled as a single object.

\begin{table*}[t]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ |c |c |c| c| c| c| c| c|c |c |c| c| c| c|}
\hline
& Body Text & Equation & Figure & Figure Caption & Other & Page Footer & Page Header&Reference Text& Section Header & Table & Table Caption & Total \\
\hline
Train & 6,578 & 1,115 & 1,384 & 1,285 & 359 & 907 & 2,765 & 496 & 3,227 & 767 & 763 & 19,646\\
\hline
Test & 1,258 & 272 & 276 & 274 & 64 & 206 & 533 & 80 & 580 & 172 & 170 & 3,885\\
\hline
\end{tabular}}
\caption{Class counts for Geosciences dataset}
\label{table:class_counts}
\end{center}
\end{table*}






==> expsetup.tex <==
We compare our model to state of the art models for page object detection. Page object detection models can be roughly divided into those based off of Faster-RCNN, and those based off of the original R-CNN. We compare to our implementations of both.

\textbf{Faster-RCNN}: A Resnet-50 convolutional map (with Feature Pyramid Network) of the entire image is produced, which is passed to a region proposal network (RPN). The RPN generates proposals. Our implementation then uses the ROI Align method from Mask-RCNN to map features from the original convolutional map to the proposals (as opposed to the original ROI Pool mechanism from Fast-RCNN). The proposal feature map is then passed to classification and regression heads for final output. This model is derived from a Tensorflow implementation of Mask-RCNN, from which we drop the branch that produces masks over proposals. For the RPN, we define anchor sizes of [64, 128, 256, 512, 1024] and aspect ratios of [0.5, 1, 2]. 

\textbf{R-CNN}: State of the art methods for page object detection generally have performed architecture search over the classification head of the original R-CNN, paired with some document segmentation algorithm to produce proposals. We compare against this class of model by using a Resnet-50 backbone to produce a convolutional map for each cropped and warped proposal. We then pass this to the classification head of Faster-RCNN to produce a class output. No regression over the final box is performed. We implement this model in PyTorch. For this model we use the same grid proposals that we generate for Attentive-RCNN.

We tune the hyperparameters of all three models by partitioning the training set into a training and validation set (80:20 split) and optimizing results over the validation set. We then use these hyperparameters to train over the entire original training set. All backbones are pretrained on ImageNet using weights available from PyTorch and Tensorflow depending on model implementation.



==> metrics.tex <==
We report standard VOC2012 average precision metrics for our Geoscience dataset experiments, with predictions ranked by classification score. If postprocessing is applied and multiple proposals are grouped, the highest score of the group is applied to the newly created output.

From an information retrieval standpoint, average precision does not tell the whole story. Especially with grid segmentation, where all pixels on the page are generally part of a proposal, we are also interested in the overall $F_1$ retrieval metric instead of a summary of the precision-recall curve. We define our end to end $F_1$ terms as follows:

\textbf{True Positive:} Any proposal with above 0.8 intersection over union (IoU) with a ground truth box, and a correct class assignment. Only one true positive proposal allowed per ground truth object

\textbf{False Positive:} Any proposal with above 0.8 IoU with a ground truth box, but an incorrect class assignment, or a proposal that has 0.7 IoU with a ground truth box for which there is already a match.

\textbf{False Negative:} Any ground truth target for which no matched ($>0.8$ IoU) proposal correctly classifies the target, and any ground truth target not matched to a proposed region.

On the ICDAR dataset, we focus on the classification task: given a matching ground truth target ($>0.8$ IoU), does the model correctly identify its class. We present confusion matrices to show the number of objects retrieved from the dataset.

==> postprocessing.tex <==
After final classification, we further refine our results by doing a postprocessing step.
First, as noted in [ALLENAI PAPER], figure and table Captions are easy to classify if the text within a proposal is available. Because we assume pdf metadata is not necessarily available, we run Tesseract OCR over each proposal. If the first token of the OCR output is \textit{fig} or \textit{figure} and the class is not a figure, we change it to Figure Caption. If the first token of the OCR output is \textit{table}, \textit{tab} or \textit{tbl} and the class is not a table, we change it to table caption.

Secondly, we note previously that our proposals tend to decompose objects that separate their content by whitespace into sub-objects, namely figures and tables. A single figure is labeled by the heuristic of a one to one mapping with a corresponding figure caption. Groups of divided sub-figures need to be properly merged into a single figure. Similarly, tables are sometimes decomposed into the table's cells that need to be merged to constitute a single table.

To resolve this situation, we merge figure and table neighborhoods. For each pair of figures or tables on a page, we take a bounding box over their union. If the union does not overlap with any other objects on the page, we replace the individual bounding boxes with their union bounding box. For tables, we more aggressively merge, allowing merges that overlap with any class except body text or captions. Any object that does overlap with the resulting table object is dropped.


==> proposal.tex <==
We first begin by producing proposals over the document. Scientific papers, regardless of origin or journal, generally adhere to some regular grid structure. Finding proposals over the document, then, is finding an appropriately sized grid.

We preprocess each image for proposal generation by converting each image to a binary map. We balance the margins of the binary map by checking the distance from each side of the page to the nearest pixel. If a side is shorter by distance $d$, we remove $d$ pixel columns from the opposite side.

We next divide each map into rows. For some row height $R$, we find all blank rows of height at least $R$. For our experiments, we set $R$ to 15 pixels. For each row between the found blank rows, we now detect whether the row can be divided into 1-3 columns. For each column number $c$, find $c-1$ division lines that divide the row into $c$ columns. If a division line intersects with a non-white pixel, we check the next column number. For all valid divisions, we take the maximum column number and split the row into that number columns. For each row-column cell, we divide the cell into rows again using the same row division process.

Finally, we refine each cell by finding all 8-connected components within the cell, filtering connected components that are too small, then taking the minimum bounding box encapsulating all connected components that remain.

Because of discrepancies between page layouts, $R$ is sometimes too low and overzealously divides cells. As a simple way to mitigate dividing a page into page lines, we check the average height of all final rows. If the average height is less than $3R$, we redivide the page, doubling $R$ for the new iteration. Our final result is a grid of proposals, each ensured not to have any overlap from another, but still approximately containing a page element.

Objects that naturally contain white space to separate their content, such as tables, are often decomposed into sub-objects by this algorithm. If these sub-objects are successfully classified as their overall object class, our post processing is then able to merge neighboring cells together based on their class.
